A Single-Loop Robust Policy Gradient Method for Robust Markov Decision Processes

Robust Markov Decision Processes (RMDPs) have recently been recognized as a valuable and promising approach to discovering a policy with creditable performance, particularly in the presence of a dynamic environment and estimation errors in the transition matrix due to limited data. Despite extensive exploration of dynamic programming algorithms for solving RMDPs, there has been a notable upswing in interest in developing efficient algorithms using the policy gradient method. In this paper, we propose the first single-loop robust policy gradient (SRPG) method with the global optimality guarantee for solving RMDPs through its minimax formulation. Moreover, we complement the convergence analysis of the nonconvex-nonconcave min-max optimization problem with the objective function's gradient dominance property, which is not explored in the prior literature. Numerical experiments validate the efficacy of SRPG, demonstrating its faster and more robust convergence behavior compared to its nested-loop counterpart.

==> flowchart.tex <==


\begin{figure}[h]
\centering

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.63,xscale=0.9]
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.63,xscale=0.9]
%uncomment if require: \path (0,959); %set diagram left start at 0, and has height of 959

%Rounded Rect [id:dp15844754527921] 
\draw   (566.43,167.39) .. controls (566.43,152.69) and (578.34,140.79) .. (593.03,140.79) -- (672.83,140.79) .. controls (687.52,140.79) and (699.43,152.69) .. (699.43,167.39) -- (699.43,638.61) .. controls (699.43,653.31) and (687.52,665.21) .. (672.83,665.21) -- (593.03,665.21) .. controls (578.34,665.21) and (566.43,653.31) .. (566.43,638.61) -- cycle ;
%Shape: Rectangle [id:dp8691182137908062] 
\draw   (578.27,314.79) -- (688.19,314.79) -- (688.19,396.79) -- (578.27,396.79) -- cycle ;
%Shape: Rectangle [id:dp733736908632362] 
\draw   (569.43,414.71) -- (695.43,414.71) -- (695.43,512.79) -- (569.43,512.79) -- cycle ;
%Shape: Rectangle [id:dp5342543038649958] 
\draw   (577.43,531.79) -- (684.82,531.79) -- (684.82,608.79) -- (577.43,608.79) -- cycle ;
%Rounded Rect [id:dp4288385356094886] 
\draw   (6.43,162.93) .. controls (6.43,148.91) and (17.8,137.54) .. (31.82,137.54) -- (536.04,137.54) .. controls (550.06,137.54) and (561.43,148.91) .. (561.43,162.93) -- (561.43,646.25) .. controls (561.43,660.27) and (550.06,671.64) .. (536.04,671.64) -- (31.82,671.64) .. controls (17.8,671.64) and (6.43,660.27) .. (6.43,646.25) -- cycle ;
%Shape: Rectangle [id:dp4166569186614515] 
\draw   (198.59,144.86) -- (289.86,144.86) -- (289.86,210.73) -- (198.59,210.73) -- cycle ;
%Shape: Rectangle [id:dp01685094982167379] 
\draw   (329.25,144.86) -- (403.86,144.86) -- (403.86,211.88) -- (329.25,211.88) -- cycle ;
%Shape: Rectangle [id:dp03213028924773664] 
\draw   (436.72,143.86) -- (519.86,143.86) -- (519.86,213.86) -- (436.72,213.86) -- cycle ;
%Shape: Rectangle [id:dp3094679650225063] 
\draw   (40.68,144.86) -- (157.86,144.86) -- (157.86,213.86) -- (40.68,213.86) -- cycle ;

%Shape: Rectangle [id:dp21334288553679337] 
\draw   (120.54,244.38) -- (218.86,244.38) -- (218.86,289.86) -- (120.54,289.86) -- cycle ;
%Shape: Rectangle [id:dp279996618409561] 
\draw   (250.36,245.36) -- (333.86,245.36) -- (333.86,291.86) -- (250.36,291.86) -- cycle ;
%Shape: Rectangle [id:dp9644776023201413] 
\draw   (353.96,244.9) -- (463.86,244.9) -- (463.86,294.86) -- (353.96,294.86) -- cycle ;
%Shape: Rectangle [id:dp9358317101562688] 
\draw   (78.19,338.5) -- (192.86,338.5) -- (192.86,412.86) -- (78.19,412.86) -- cycle ;
%Shape: Rectangle [id:dp2436002675207296] 
\draw   (234.65,335.43) -- (343.14,335.43) -- (343.14,425.5) -- (234.65,425.5) -- cycle ;
%Shape: Rectangle [id:dp15286027963075766] 
\draw   (384.14,336.93) -- (483.14,336.93) -- (483.14,409.93) -- (384.14,409.93) -- cycle ;
%Shape: Rectangle [id:dp8310471539202988] 
\draw   (98.49,470.79) -- (244.8,470.79) -- (244.8,533.05) -- (98.49,533.05) -- cycle ;
%Shape: Rectangle [id:dp1107824965185693] 
\draw   (291.62,471.79) -- (427.78,471.79) -- (427.78,536.69) -- (291.62,536.69) -- cycle ;
%Shape: Rectangle [id:dp2401856135676741] 
\draw   (200.82,575.96) -- (402.1,575.96) -- (402.1,640.86) -- (200.82,640.86) -- cycle ;
%Curve Lines [id:da9642685704744691] 
\draw    (242.86,214.86) .. controls (207.88,230.35) and (248.52,313.39) .. (259.01,329.69) ;
\draw [shift={(260.02,331.19)}, rotate = 234.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da3631303206240084] 
\draw    (368.15,212.86) .. controls (343.91,261.02) and (335.15,311.41) .. (332.99,328.28) ;
\draw [shift={(332.75,330.22)}, rotate = 276.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da829383621461691] 
\draw    (376.37,212.39) .. controls (597.1,242.57) and (564.12,484.08) .. (429.65,505.5) ;
\draw [shift={(429.65,505.5)}, rotate = 350.95] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da8773723662462134] 
\draw    (92.86,220.86) .. controls (2.37,368.88) and (57.53,620.41) .. (289.62,535.69) ;
\draw [shift={(289.62,535.69)}, rotate = 159.95] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp12462060969039457] 
\draw   (8.14,698.59) .. controls (8.14,687.77) and (16.91,679) .. (27.73,679) -- (675.56,679) .. controls (686.37,679) and (695.14,687.77) .. (695.14,698.59) -- (695.14,757.34) .. controls (695.14,768.16) and (686.37,776.93) .. (675.56,776.93) -- (27.73,776.93) .. controls (16.91,776.93) and (8.14,768.16) .. (8.14,757.34) -- cycle ;
%Shape: Rectangle [id:dp7104399375528889] 
\draw   (135.98,686) -- (284.94,686) -- (284.94,764.93) -- (135.98,764.93) -- cycle ;
%Shape: Rectangle [id:dp4290311075399704] 
\draw   (320.52,683.93) -- (489.49,683.93) -- (489.49,770.93) -- (320.52,770.93) -- cycle ;
%Shape: Rectangle [id:dp292974421310056] 
\draw   (524.14,689.21) -- (653.14,689.21) -- (653.14,766.21) -- (524.14,766.21) -- cycle ;
%Curve Lines [id:da005984922511056201] 
\draw    (573.43,354.64) .. controls (555.61,329.89) and (397.63,312.98) .. (352.75,332.05) ;
\draw [shift={(351.43,332.64)}, rotate = 335.06] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da719321959127406] 
\draw    (562,463.29) .. controls (542.62,454.45) and (449.32,559.23) .. (408.64,586.55) ;
\draw [shift={(407.43,587.36)}, rotate = 326.98] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da4039826238412938] 
\draw    (566.43,566.36) .. controls (531.95,565.37) and (426.37,246.57) .. (406.97,207.38) ;
\draw [shift={(406.14,205.79)}, rotate = 61.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da9467356414883719] 
\draw    (406.86,625.14) .. controls (584.73,629.87) and (575.52,664.23) .. (574.25,680.3) ;
\draw [shift={(574.14,682.21)}, rotate = 271.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da8306672878406243] 
\draw    (562,463.29) .. controls (511.72,468.65) and (431.97,649.74) .. (421.52,676.4) ;
\draw [shift={(420.86,678.14)}, rotate = 290.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9688614028041604] 
\draw    (196,180) -- (163.14,179.8) ;
\draw [shift={(161.14,179.79)}, rotate = 0.35] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6469120421264931] 
\draw    (292.14,180.79) -- (325.14,180.79) ;
\draw [shift={(327.14,180.79)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8277460775229735] 
\draw    (407.14,182.79) -- (431.14,182.79) ;
\draw [shift={(433.14,182.79)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4520721696353327] 
\draw    (228.14,213.93) -- (174.93,241.02) ;
\draw [shift={(173.14,241.93)}, rotate = 333.02] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da043840854393447204] 
\draw    (262.14,213.93) -- (283.87,240.38) ;
\draw [shift={(285.14,241.93)}, rotate = 230.6] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5643214687738887] 
\draw    (289.86,210.73) -- (382.24,241.3) ;
\draw [shift={(384.14,241.93)}, rotate = 198.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5491209289924588] 
\draw    (143.14,290.93) -- (126.64,329.59) ;
\draw [shift={(125.86,331.43)}, rotate = 293.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da03209809093670324] 
\draw    (250.36,291.86) -- (139.99,337.17) ;
\draw [shift={(138.14,337.93)}, rotate = 337.68] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4093964361078426] 
\draw    (353.96,294.86) -- (178.08,338.45) ;
\draw [shift={(176.14,338.93)}, rotate = 346.08] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da627385999775943] 
\draw    (134,415.14) -- (289.74,471.12) ;
\draw [shift={(291.62,471.79)}, rotate = 199.77] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1946760081752239] 
\draw    (287.14,424.93) -- (351.49,468.8) ;
\draw [shift={(353.14,469.93)}, rotate = 214.29] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6985098488121555] 
\draw    (427,410.14) -- (376.47,467.43) ;
\draw [shift={(375.14,468.93)}, rotate = 311.42] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8840615599052328] 
\draw    (246.14,506.64) -- (288.14,506.64) ;
\draw [shift={(290.14,506.64)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4866803825044057] 
\draw    (329.14,536.64) -- (329.14,573.64) ;
\draw [shift={(329.14,575.64)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5818790756875722] 
\draw    (287.14,730.79) -- (315.14,730.79) ;
\draw [shift={(317.14,730.79)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1800439497183266] 
\draw    (493.14,729.79) -- (521.14,729.79) ;
\draw [shift={(523.14,729.79)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (602.82,259) node [anchor=north west][inner sep=0.75pt]   [align=left] {Auxillary\\Results};
% Text Node
\draw (21.74,568.55) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{53.76pt}\setlength\topsep{0pt}
\begin{center}
Proof \\Section 4.2
\end{center}

\end{minipage}};
% Text Node
\draw (359.96,244.9) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{66.66pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma C.7}\\{\footnotesize Proximal Descent}
\end{center}

\end{minipage}};
% Text Node
\draw (597.43,327.97) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{46.71pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma B.1 }\\{\footnotesize Gradient }\\{\footnotesize Dominance}
\end{center}

\end{minipage}};
% Text Node
\draw (436.72,146.86) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{52.32pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Lemma C.3 }\\{\scriptsize Smoothness of }\\{\scriptsize Dual function}
\end{center}

\end{minipage}};
% Text Node
\draw (126.54,244.38) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{58.05pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma C.5}\\{\footnotesize Primal Descent}
\end{center}

\end{minipage}};
% Text Node
\draw (203.64,145.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{55.49pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Lemma C.1 }\\{\scriptsize Strong convexity}\\{\scriptsize Smoothness}
\end{center}

\end{minipage}};
% Text Node
\draw (335.25,145.1) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{45.97pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Lemma C.2 }\\{\scriptsize Lipschitz type}\\{\scriptsize Error Bound}
\end{center}

\end{minipage}};
% Text Node
\draw (114.06,469.98) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{74.41pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Lemma C.9}\\{\scriptsize Sufficient Condition for}\\{\scriptsize Stationary Point}
\end{center}

\end{minipage}};
% Text Node
\draw (82.92,341.41) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{70.01pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Proposition 4.1 }\\{\footnotesize (Proposition C.1)}\\{\footnotesize Lyapunov Descent}
\end{center}

\end{minipage}};
% Text Node
\draw (239.92,333.35) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{66.52pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Proposition 4.2 }\\{\footnotesize (Proposition C.2)}\\{\footnotesize Upper Bound of }\\{\footnotesize Interference Term}
\end{center}

\end{minipage}};
% Text Node
\draw (388.54,342.39) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{62.15pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma C.8}\\{\footnotesize Upper Bound of }\\{\footnotesize Initial Value}
\end{center}

\end{minipage}};
% Text Node
\draw (314.5,471.98) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{60.65pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Theorem 4.1 }\\{\scriptsize (Theorem C.1)}\\{\scriptsize Stationary Results}
\end{center}

\end{minipage}};
% Text Node
\draw (225.04,575.15) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{106.59pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Theorem 4.2 }\\{\footnotesize (Theorem C.2)}\\{\footnotesize Global Convergence Results}
\end{center}

\end{minipage}};
% Text Node
\draw (257.13,245.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{46.27pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma C.6}\\{\footnotesize Dual Ascent}
\end{center}

\end{minipage}};
% Text Node
\draw (585.63,419) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{65.78pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Theorem 3.2 }\\{\footnotesize Moreau envelope}\\{\footnotesize Gradient }\\{\footnotesize Dominance}
\end{center}

\end{minipage}};
% Text Node
\draw (595.59,539) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{48.08pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma 3.1 }\\{\footnotesize Full }\\{\footnotesize Smoothness}
\end{center}

\end{minipage}};
% Text Node
\draw (39.45,696.34) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{53.76pt}\setlength\topsep{0pt}
\begin{center}
Proof \\Section 4.3
\end{center}

\end{minipage}};
% Text Node
\draw (157.01,692.97) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{68.05pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma C.10 }\\{\footnotesize Moreau envelope }\\{\footnotesize Property}
\end{center}

\end{minipage}};
% Text Node
\draw (323.94,692.97) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{108.41pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Lemma 4.2 }\\{\footnotesize (Lemma C.11) }\\{\footnotesize Regional Exponential Growth}
\end{center}

\end{minipage}};
% Text Node
\draw (544.7,694.93) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{60.78pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Proposition 4.3}\\{\footnotesize (Proposition C.3) }\\{\footnotesize Changing rate}
\end{center}

\end{minipage}};
% Text Node
\draw (53.68,147.24) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{62.24pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Lemma C.4 }\\{\scriptsize Correlation among}\\{\scriptsize Iterative Sequence}
\end{center}

\end{minipage}};


\end{tikzpicture}
\caption{Flowchart of proof process}
\end{figure}
